Cloudy in the microcalorimeter era: improved energies for K$\alpha$ transitions

X-ray missions with microcalorimeter technology will resolve spectral features with unprecedented detail. In this work, we improve the H-like K$\alpha$ energies for elements between 6 $\leq Z \leq$ 30 for the release version of the spectral simulation code Cloudy to match laboratory energies. We update the ionization potential ($I_{\rm ion}$) for these elements and add a fourth-order polynomial to the level energy difference. This brings the release version of Cloudy into a near-perfect agreement with NIST. The updated energies are $\sim$ 15-4000 times more precise than that of the current release version of Cloudy (C17.02). These new changes will be a part of the next update to the release version, C17.03.

==> macros.tex <==
% 20 06 24, copied from  aastex63.cls

%% need this change so that it works correctly in tables:
{\catcode`\$=\active
\gdef\nodata{ ~$\cdots$~ }}% 

%\newcommand\diameter{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}% 

 

% some names we use
\newcommand{\Cloudy}{\textsc{Cloudy}}
\newcommand{\Hazy}{\textsc{Hazy}}
\newcommand{\cdCommand}[1]{\textbf{#1}}
\newcommand{\cdVariable}[1]{\emph{#1}}
\newcommand{\cdSectionTitle}[1]{\emph{#1}}
\newcommand{\cdFilename}[1]{\texttt{#1}}
\newcommand{\cdRoutine}[1]{\emph{#1}}
\newcommand{\cdTerm}[1]{\textbf{\emph{#1}}}
\newcommand{\cdMono}[1]{\texttt{#1}}
\newcommand{\fixit}[1]{\textbf{FIXIT: #1}}
\font\manual=manfnt at 7pt \def\dbend{\hbox{\raise0.9ex\hbox{\manual\char127\hspace{0.6em}}}}
\newcommand{\experimental}{\texorpdfstring{\dbend}{??}}

% or symbol provided by Will H
\newcommand\OR{\texorpdfstring{\ensuremath{\vert}}{|}}

% Matt's 1.23\e{-2} 
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}


% \ion from Will, replace AAS version
\newcommand\Ion[2]{\ensuremath{\mathrm{#1\,\scriptstyle #2}}}

% macro sometimes found in ADS bibtex entries

% ion is in the aas style
\newcounter{INTERNALionstage}
\providecommand{\ion}[2]{% replace the aastex version
  \setcounter{INTERNALionstage}{#2}%
  \Ion{#1}{\Roman{INTERNALionstage}}}

\providecommand{\red}[1]{{\color{red}#1}}

% Will's todo and done macros
%\newcommand\TODO[1]{\textbf{\boldmath [#1]}}
\newcommand{\TODO}[1]{\textcolor{red}{{\textbf{\boldmath [#1]}}}}
\newcommand\DONE[1]{{\color{green!50!gray} \textbf{DONE}} {\color{white!80!black!80!green} #1}}

\newcommand{\Av}{A$_{\rm V}$}

\def\gtsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\Msunpyr{M$_{\odot}\,$yr$^{-1}$}
\def\Msun{M$_{\odot}$}
%       Based on PATs UNITS.TEX with some additions
%
%       Simple units
%
\def\A{{\rm\thinspace \AA}}
\def\cm{{\rm\thinspace cm}}
\def\as{{\rm\thinspace arcsec}}
\def\erg{{\rm\thinspace erg}}
\def\eV{{\rm\thinspace eV}}
\def\g{{\rm\thinspace g}}
\def\ga{{\rm\thinspace gauss}}
\def\hr{{\rm\thinspace hr}}
\def\Hz{{\rm\thinspace Hz}}
\def\K{{\rm\thinspace K}}
\def\keV{{\rm\thinspace keV}}
\def\km{{\rm\thinspace km}}
\def\kpc{{\rm\thinspace kpc}}
\def\Lsun{\mbox{$\rm\thinspace L_{\odot}$}}
\def\m{{\rm\thinspace m}}
\def\MeV{{\rm\thinspace MeV}}
\def\mJy{{\rm\thinspace mJy}}
\def\micron{\hbox{$\mu$m}}
\def\Mpc{{\rm\thinspace Mpc}}
\def\Msun{\mbox{$\rm\thinspace M_{\odot}$}}
\def\nm{{\rm\thinspace nm}}
\def\pc{{\rm\thinspace pc}}
\def\ps{{\rm\thinspace s^{-1}}}
\def\pcc{{\rm\thinspace cm^{-3}}}
\def\Ryd{{\rm\thinspace Ryd}}
\def\s{{\rm\thinspace s}}
\def\sr{{\rm\thinspace sr}}
\def\W{{\rm\thinspace W}}
\def\yr{{\rm\thinspace yr}}
%
%       Compound units
%
\def\keVscm{\mbox{$\keV\cm^{2}\,$}}
\def\cmps{\mbox{$\cm\s^{-1}\,$}}
\def\cmpss{\mbox{$\cm\s^{-2}\,$}}
\def\ccmps{\mbox{$\cm^{3}\s^{-1}\,$}}
\def\ergpccmps{\mbox{$\erg\cm^{-3}\s^{-1}\,$}}
\def\ergpg{\mbox{$\erg\g^{-1}\,$}}
\def\ergpscm{\mbox{$\erg\cm^{-2}\,$}}
\def\ergpscmps{\mbox{$\erg\cm^{-2}\s^{-1}\,$}}
\def\ergpscmpspsas{\mbox{$\erg\cm^{-2}\s^{-1}\as^{-2}\,$}}
\def\ergpscmpspa{\mbox{$\erg\cm^{-2}\s^{-1}\A^{-1}\,$}}
\def\ergps{\mbox{$\erg\s^{-1}\,$}}
\def\gpcm{\mbox{$\g\cm^{-3}\,$}}
\def\gpcmps{\mbox{$\g\cm^{-3}\s^{-1}\,$}}
\def\gps{\mbox{$\g\s^{-1}\,$}}
\def\uJy{\mbox{$\mu${\rm Jy}}}
\def\kmps{\mbox{$\km\ps\,$}}
\def\kmpspMpc{\mbox{$\kmps\Mpc^{-1}\,$}}
\def\Lsunppc{\mbox{$\Lsun\pc^{-3}\,$}}
\def\Msunpc{\mbox{$\Msun\pc^{-3}\,$}}
\def\Msunpkpc{\mbox{$\Msun\kpc^{-1}\,$}}
\def\Msunppc{\mbox{$\Msun\pc^{-3}\,$}}
\def\Msunppcpyr{\mbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\def\Msunpyr{\mbox{$\Msun\yr^{-1}\,$}}
\def\Msunpyrpkpc{\mbox{$\Msun\yr^{-1}\kpc^{-1}\,$}}
\def\ps{\mbox{$\s^{-1}\,$}}
\def\pscm{\mbox{$\cm^{-2}\,$}}
\def\psm{\mbox{$\m^{-2}\,$}}
\def\pccm{\mbox{$\cm^{-3}\,$}}
\def\pscm{\mbox{$\cm^{-2}\,$}}
\def\pscmps{\mbox{$\cm^{-2}\, \s^{-1}\,$}}
\def\pcm{\mbox{$\m^{-3}\,$}}
\def\pccmK{\mbox{$\cm^{-3}\K$}}
\def\pcmK{\mbox{$\m^{-3}\K$}}
\def\pressure{\mbox{$\g\, \cm^{-1}\, \s^{-2}\,$}}
\def\pyr{\mbox{$\yr^{-1}\,$}}
\def\pyrppc{\mbox{$\yr^{-1}\pc^{-1}\,$}}
\def\scm{\mbox{$\cm^{2}\,$}}
\def\Wpsm{\mbox{$\W\psm\,$}}
\def\Wpscm{\mbox{$\W\pscm\,$}}
\def\WHz{\mbox{$\W\Hz\,$}}
%
% spectral lines
%
\def\la{\mbox{{\rm L}$\alpha$}}
\def\pa{\mbox{{\rm P}$\alpha$}}
\def\ha{\mbox{{\rm H}$\alpha$}}
\def\hb{\mbox{{\rm H}$\beta$}}
\def\hi{\mbox{{\rm H~{\sc i}}}}
\def\hii{\mbox{{\rm H~{\sc ii}}}}
\def\hei{\mbox{{\rm He~{\sc i}}}}
\def\heii{\mbox{{\rm He~{\sc ii}}}}
\def\ci{\mbox{{\rm C~{\sc i}}}}
\def\cii{\mbox{{\rm C~{\sc ii}}}}
\def\ciii{\mbox{{\rm C~{\sc iii}}}}
\def\civ{\mbox{{\rm C~{\sc iv}}}}
\def\ni{\mbox{{\rm N~{\sc i}}}}
\def\nii{\mbox{{\rm N~{\sc ii}}}}
\def\oi{\mbox{{\rm O~{\sc i}}}}
\def\oii{\mbox{{\rm O~{\sc ii}}}}
\def\oiii{\mbox{{\rm O~{\sc iii}}}}
\def\neii{\mbox{{\rm Ne~{\sc ii}}}}
\def\neiii{\mbox{{\rm Ne~{\sc iii}}}}
\def\nev{\mbox{{\rm Ne~{\sc v}}}}
\def\mgii{\mbox{{\rm Mg~{\sc ii}}}}
\def\cliii{\mbox{{\rm Cl~{\sc iii}}}}
\def\sii{\mbox{{\rm S~{\sc ii}}}}
\def\siii{\mbox{{\rm S~{\sc iii}}}}
\def\ariii{\mbox{{\rm Ar~{\sc iii}}}}
\def\caii{\mbox{{\rm Ca~{\sc ii}}}}
\def\fei{\mbox{{\rm Fe~{\sc i}}}}
\def\feii{\mbox{{\rm Fe~{\sc ii}}}}
\def\feiii{\mbox{{\rm Fe~{\sc iii}}}}
\def\feiv{\mbox{{\rm Fe~{\sc iv}}}}
\def\fev{\mbox{{\rm Fe~{\sc v}}}}
\def\fevi{\mbox{{\rm Fe~{\sc vi}}}}
\def\fevii{\mbox{{\rm Fe~{\sc vii}}}}
\def\feviii{\mbox{{\rm Fe~{\sc viii}}}}
\def\feix{\mbox{{\rm Fe~{\sc ix}}}}
\def\fex{\mbox{{\rm Fe~{\sc x}}}}
\def\fexi{\mbox{{\rm Fe~{\sc xi}}}}
\def\fexii{\mbox{{\rm Fe~{\sc xii}}}}
\def\fexiii{\mbox{{\rm Fe~{\sc xiii}}}}
\def\fexiv{\mbox{{\rm Fe~{\sc xiv}}}}
\def\fexv{\mbox{{\rm Fe~{\sc xv}}}}
\def\fexvi{\mbox{{\rm Fe~{\sc xvi}}}}
\def\fexvii{\mbox{{\rm Fe~{\sc xvii}}}}
\def\fexviii{\mbox{{\rm Fe~{\sc xviii}}}}
\def\fexix{\mbox{{\rm Fe~{\sc xix}}}}
\def\fexx{\mbox{{\rm Fe~{\sc xx}}}}
\def\fexxi{\mbox{{\rm Fe~{\sc xxi}}}}
\def\fexxii{\mbox{{\rm Fe~{\sc xxii}}}}
\def\fexxiii{\mbox{{\rm Fe~{\sc xxiii}}}}
\def\fexxiv{\mbox{{\rm Fe~{\sc xxiv}}}}
\def\fexxv{\mbox{{\rm Fe~{\sc xxv}}}}
\def\fexxvi{\mbox{{\rm Fe~{\sc xxvi}}}}
%
% types of baryons
\def\water{\mbox{{\rm H}$_2${\rm O}}}
\def\CO{\mbox{{\rm CO}}}
\def\OH{\mbox{{\rm OH}}}
\def\htwo{\mbox{{\rm H}$_2$}}
\def\hone{\mbox{{\rm H}$^0$}}
\def\h0{\mbox{{\rm H}$^0$}}
%
% \def\H{\mbox{{\rm H}}}
%
\def\hplus{\mbox{{\rm H}$^+$}}
\def\hminus{\mbox{{\rm H}$^-$}}
% cannot have numbers in names, so cap Oh represents zero
\def\hO{\mbox{{\rm H}$^0$}}
\def\heO{\mbox{{\rm He}$^0$}}
\def\heo{\mbox{{\rm He}$^0$}}
\def\heplus{\mbox{{\rm He}$^+$}}
\def\hePP{\mbox{{\rm He}$^{2+}$}}
\def\cO{\mbox{{\rm C}$^0$}}
\def\cplus{\mbox{{\rm C}$^+$}}
%
\def\Hrec{\mbox{${\rm H}_{rec}$}}
%\def\Hrec{\mbox{$H_{rec}$}}
\def\centreline{\centerline}
%
% Nina
\DeclareMathAlphabet{\vib}{OML}{cmm}{m}{it}
% From Glenn
\newcommand*{\satellite}[1]{\textit{#1}}
\newcommand*{\xmm}{\satellite{XMM-Newton}}
\newcommand*{\chandra}{\satellite{Chandra}}
\newcommand*{\asca}{\satellite{ASCA}}
\newcommand*{\rosat}{\satellite{ROSAT}}
\newcommand*{\prog}[1]{\textsc{#1}}
%% For kb, mH. etc. Italic with non-italic subscript.
\newcommand*{\mysub}[2]{\ensuremath{#1_{\mathrm{#2}}}}

